Long-living Service for Cooperative Knowledge Use in Decentralized Data Stores

Personal Data Stores (PDS) like SoLiD is an emerging data and knowledge management solution in recent years. They promise to give back ownership and control of data to the user, and provide protocols for developers to build applications using the data. However, existing Solid-based applications often focus on using a single-user's data. In this article, we use a simple but realistic calendar-and-meeting-scheduling scenario to demonstrate the feasibility and design considerations for enabling cooperative data-use across multiple users' SoLiD Pods. This scenario identifies the bottleneck for certain cooperative use cases, namely those involving offline-changing and synchronization of knowledge information. We demonstrate a viable approach to mediate this issue, introducing a long-living thin service, the orchestrator. We describe our implementation and discuss its applicability to other ecosystems. We conclude by discussing the implication of such services, in particular their risks and challenges for building decentralised applications.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto
